Robust Tuning Datasets for Statistical Machine Translation

We explore the idea of automatically crafting a tuning dataset for Statistical Machine Translation (SMT) that makes the hyper-parameters of the SMT system more robust with respect to some specific deficiencies of the parameter tuning algorithms. This is an under-explored research direction, which can allow better parameter tuning. In this paper, we achieve this goal by selecting a subset of the available sentence pairs, which are more suitable for specific combinations of optimizers, objective functions, and evaluation measures. We demonstrate the potential of the idea with the pairwise ranking optimization (PRO) optimizer, which is known to yield too short translations. We show that the learning problem can be alleviated by tuning on a subset of the development set, selected based on sentence length. In particular, using the longest 50% of the tuning sentences, we achieve two-fold tuning speedup, and improvements in BLEU score that rival those of alternatives, which fix BLEU+1's smoothing instead.

==> results.tex <==


%\subsection{Datasets}
\label{datasets}

We experiment with single-reference and multi-reference tuning and testing datasets for two language pairs:
Spanish-English and Arabic-English.

For Spanish-English, we use the single-reference datasets newstest2008, newstest2009, newstest2010, newstest2011
from the WMT~2012, Workshop on Machine Translation Evaluation.\footnote{\texttt{www.statmt.org/wmt12/}}

For Arabic-English, we use the multi-reference datasets MT04, MT05, MT06, and MT09
from the NIST 2012 OpenMT Evaluation.\footnote{\texttt{www.nist.gov/itl/iad/mig/openmt12.cfm}}.
For this language pair, we further experiment with single-reference versions of these datasets,
where we use the first (default) reference only.

In addition to the above datasets,
we further constructed tuning sets of different source-side sentence lengths: \emph{short}, \emph{middle} and \emph{long}.
Given a dataset, we selected 50\% of its sentence pairs:
the \emph{shortest} 50\%, the \emph{middle} 50\%, or the \emph{longest} 50\%.
This yielded datasets with the same number of sentences but different number of words,
e.g., for our Arabic-English datasets, \emph{longest} has about twice as many words as \emph{middle},
and about four times as many words as \emph{shortest}.

%\textbf{Hmm, we had something special about the sampling of sentences to avoid bias? Should we mention it?}


\subsection{Experimental Setup}

We experimented with the phrase-based SMT model \cite{Koehn:2003:SPT} as implemented in the Moses toolkit \cite{Moses:2007}.
We trained the Arabic-English system on all training data from NIST 2012 except for the UN corpus.

For training the Spanish-English system, we used all the data available for the WMT12 evaluation, again except for the UN data.

We tokenized and truecased the English and the Spanish side of all bitexts and also the monolingual data for language modeling
using the standard tokenizer of Moses.
We segmented the words on the Arabic side using the MADA ATB segmentation scheme \cite{MADA}.
We built our phrase tables using the Moses pipeline with max-phrase-length 7 and Kneser-Ney smoothing.
We also built a lexicalized reordering model \cite{IWSLT:2005}: \emph{msd-bidirectional-fe}.
We used a 5-gram language model trained on GigaWord v.5 with Kneser-Ney smoothing using KenLM \cite{kenlm}.

On tuning and testing, we dropped unknown words for Arabic-English, and we used monotone-at-punctuation decoding for Spanish-English.


We performed tuning using two parameter optimization algorithms for statistical machine translation: MERT and PRO.
We used the standard implementation of MERT from the Moses toolkit,
but a slightly modified, fixed version of PRO, as recommended by \newcite{nakov-guzman-vogel:2013:Short},
which solves issues with PRO's instability when tuning on the \emph{long} sentences.

%we will discuss our PRO fix and the reasons it is needed in Section~\ref{sec:discuss} below.
In order to ensure convergence, we allowed both MERT and PRO to run for up to 25 iterations (default: 16);
we further used 1000-best lists in each iteration (default: 100).

In our experiments below, we perform three reruns of parameter optimization,
tuning on each of these twelve tuning datasets;
in the figures, we plot the results of the three reruns,
while in the tables, we report BLEU averaged over the three reruns, as suggested by \newcite{clark-EtAl:2011:ACL-HLT2011} as a way to stabilize MERT.

For evaluation, we used NIST's BLEU v13a scoring tool, in case-sensitive mode.


%\subsection{Analysis of Optimization}

\begin{figure*}[htb!]
  \centering
  \includegraphics[width=0.9\linewidth]{final.figure/length_tune_hverb.pdf}

 \caption{\label{fig:tuning}
          \emph{Source-side length} vs. \emph{hypothesis verbosity} for the tuning dataset.}
%          Plotted are the results for Spanish-English (1-ref.) and Arabic-English (multi-ref and 1-ref),
%          with twelve datasets per language pair:
%          four tuning datasets, each split into three datasets (\emph{short}, \emph{middle}, and \emph{long}).
%          There are three points for each of these twelve datasets since we have three reruns.
%%          The results of tuning on the different length-bins for each of the Spanish-English WMT (newstest 2008-2011) sets are presented  on the upper half. On the lower half, we present the results of the Arabic-English NIST sets (MT04, MT05, MT06, MT09). Each point represents the hypothesis to reference ratio of the translations obtained after tuning plotted against the input source length of each dataset.
%          A regression line is added to help see the tendencies.}
 \end{figure*}


\subsection{Learning verbosity}

%In order to answer this question, we performed an in-depth analysis of the verbosity that MERT and PRO learn.
%We experimented with two language pairs and four tuning datasets per pair.  For Arabic-English, we used the multi-reference NIST datasets MT04, MT05, MT06 and MT09, while for Spanish-English, we used the single-reference WMT newstest2008, newstest2009, newstest2010, and newstest2011. From each of these datasets, we generated three new tuning datasets of varying lengths by selecting the shortest/medium/longest 50\% of its sentences. As a result, we ended up with 12 datasets per language pair.

In our first experiment, we performed parameter optimization using MERT and PRO on each dataset,
and we used the resulting parameters to translate the same dataset that we used for tuning.
The purpose of this experiment was to study the ability of the optimizers to learn the \emph{verbosity} of the tuning datasets. 
Getting the \hvb right
means that it is highly correlated with the tuning set \vb, which in turn is determined by the dataset source length.

%After optimization, we obtain a total of 24 sets of parameters (12 for MERT, 12 for PRO) for each language-pair.
%Then, we translate each tuning dataset with its corresponding set of weights,
%and we calculate the verbosity of the resulting translations.
%This procedure was performed in order to assess the ability of each optimizer to obtain reasonable parameters given a tuning set.
The results of this experiment are shown in Figure~\ref{fig:tuning}.
In each graph, there are 36 points (many of them very close and overlapping)
since we performed three reruns for each experiment with our twelve tuning datasets
(three length-based subsets for each of the four original tuning datasets).

There are several observations that we can make about the results in Figure~\ref{fig:tuning}:

(1) MERT has a fairly stable behavior with respect to the input length of the sentences in the tuning datasets. Observe how the MERT regression lines imitate those in (Fig.\ref{fig:scatter}). In fact, the correlation between the \vb and the \hvb for MERT is $r$=0.980.
PRO, on the other hand, has a harder time learning the tuning set verbosity, and the correlation with the \hvb is only $r$=0.44. Interestingly enough, its \lr exhibits a behavior that more sensitive to the input length ($r$=0.67):
on \emph{short} sentences, it learns to output translations that are slightly shorter than the reference,
and on \emph{long} sentences it yields increasingly longer translations. The dependence of PRO on source length can be related to the sentence level smoothing BLEU and the broken balance between the precision component and BP. The problem is bigger for short sentences because there is a +1 is added to smaller counts, which results on a preference for shorter translations.

(2) Looking at the impact of the number of references for Arabic-English,
we observe that having multiple references makes both MERT and PRO appear more stable,
%(maybe because the effective reference length is more permissive with more references),
% TODO: Check this with the data?
allowing them to generate hypotheses that are less spread, and closer to 1.
This can be attributed to the \emph{effective reference length},
which naturally dampens the effect of verbosity
during optimization by selecting the reference that is closest to the respective hypothesis.

%(3) When comparing the language pairs, we observe different behaviors for Arabic-English and Spanish-English:
%Arabic-English hypotheses tend to be shorter than their references,
%while those for Spanish-English are longer.
%fairly stable behavior with respect to the input length of the sentences in the tuning datasets.
%Regardless of the average source length, the resulting length ratio is close to $1$.
%(esp. when working with the multi-reference Arabic-English datasets).
%Thus, it does learn to translate with the right verbosity.

%Furthermore, this behavior changes as we increase the length of the tuning set.
%With medium-length sentences, PRO learns to generate translations that are slightly longer than the reference.
%In addition, we observe that as the input sentences get longer, the behavior of PRO becomes increasingly unstable.
%This is especially troublesome when dealing with the single-reference Spanish-English tuning datasets (see the upper right panel).
%However, this tendency is less pronounced when dealing with the multi-reference Arabic-English.

Overall, based on these experimental results,
we can conclude that MERT is capable of learning the tuning set's \emph{verbosity} more accurately than PRO.
PRO learns \emph{verbosity} that is more dependent on the \emph{source side length} of the sentences in the tuning dataset.
%This is particularly visible in the case of single-reference optimizations.

%\textbf{Do we want to suggest why this is happening? Or maybe try to speculate on this in the Discussion?}

%We should note that the inability of PRO to learn the right verbosity is not entirely surprising.
%It has been observed previously that PRO tends to generate too short translations.
%\textbf{I need to finish this paragraph.}

%Moreover, PRO shows instability in what it learns, clearly a very undesirable property of any optimizer. We will explore this behavior of PRO in more detail in Section~\ref{sec:discussion} below, where we will also suggest some possible ways to stabilize it.

%> fd<-full[full$set=="Ar-En"& full$tuner=="MERT",]


% \subsection{Translation performance}
\subsection{Performance on the Test Dataset}

In our next experiment, we study the performance of MERT and PRO
when testing on datasets that are different from the one used for tuning. First, we want to test the robustness of the parameters that were obtained under the specific conditions. Second, we want to test the whether length can be a reasonable criteria to select a tuning set.

For this purpose, we perform a grid comparison of tuning and testing on all our datasets:
we tune on each \emph{short}/\emph{middle}/\emph{long} dataset,
and we test on the remaining \emph{short}/\emph{middle}/\emph{long}/\emph{full} datasets.

The results are shown in Table~\ref{tab:bleu}.
Each cell in the table represents an average over 36 BLEU scores:
four tuning sets times three test sets times three reruns.
For example, the number 49.63 in row 1 (tuning on short), column 2 (testing on middle), corresponds to the average over
three reruns of
(i) tuning on MT04-short and testing on MT05-middle, MT06-middle, and MT09-middle,
(ii) tuning on MT05-short and testing on MT04-middle, MT06-middle, and MT09-middle,
(iii) tuning on MT06-short and testing on MT04-middle, MT05-middle, and MT09-middle,
and
(iv) tuning on MT09-short and testing on MT04-middle, MT05-middle, and MT06-middle.

The table also includes the results when \emph{testing} on the full datasets;
however, in order to avoid asymmetrical tuning conditions (in terms of number of training examples),
here we opted not to show the results for \emph{tuning} on the full dataset.



%\begin{table}[htb]
%    \centering
%    \begin{tabular}{lcccc}
%      \toprule
%       \multicolumn{5}{l}{\bf  NIST Arabic-English (multi-ref)}\\
%       \multicolumn{5}{r}{\bf \it Average BLEU on unseen test sets}\\\cmidrule{2-5}
%
%      & {\bf short} & {\bf mid} & {\bf long} & {\bf full} \\\midrule
%
%      \multicolumn{5}{l}{\bf  MERT}\\
%      tune-short &\bf{45.87} & 49.84 & 50.36 & 48.96  \\
%      tune-mid   & 45.80 & \bf{50.22} & 50.70 & 49.25  \\
%      tune-long  & \bf {45.84} &\bf{ 50.24} &\bf{50.94} & \bf{49.42}  \\
%
%      \multicolumn{5}{l}{\bf PRO}\\
%      tune-short & 45.86 & 50.01 & 50.51 & 49.14  \\
%      tune-mid & \bf{46.04*} & \bf{50.34*} & \bf{50.96*} & \bf{49.54*}  \\
%      tune-long & \it{44.02} & \it{48.07} & \it{48.71} & \it{47.54}  \\
%      \bottomrule
%      \\\toprule
%      \multicolumn{5}{l}{\bf WMT Spanish-English}\\
%      \multicolumn{5}{r}{\bf \it Average BLEU on unseen test sets}\\\cmidrule{2-5}
%
%      & {\bf short} & {\bf mid} & {\bf long} & {\bf full} \\\midrule
%      \multicolumn{5}{l}{\bf  MERT}\\
%       tune-short & 24.50 & 25.59 & 27.46 & 26.70  \\
%      tune-mid & \bf{24.61*} & \bf{25.87*} & 27.78 & \bf{27.00}  \\
%      tune-long & 24.54 & \bf{25.87*} &\bf{27.90*} & \bf{27.05*}  \\
%     \multicolumn{5}{l}{\bf PRO}\\
%
%     tune-short & \bf{24.54} & \bf{25.78} & \bf{27.83} & \bf{27.07*}  \\
%       tune-mid & 24.20 & 25.29 & 27.12 & 26.42  \\
%     tune-long & \it{22.82} & \it{23.96} & \it{25.74} & \it{25.08}  \\ \bottomrule
%
%    \end{tabular}
%    \caption{\label{tab:bleu}
%    OLD}
%\end{table}



\begin{table}[h!]
    \small
    \centering
    \begin{tabular}{lcccc}

      \toprule
       \multicolumn{5}{l}{\bf  NIST Arabic-English (multi-ref)}\\
       \multicolumn{5}{r}{\bf \it Average BLEU on unseen test sets}\\\cmidrule{2-5}

      & {\bf short} & {\bf mid} & {\bf long} & {\bf full} \\\midrule

      \multicolumn{5}{l}{\bf  MERT}\\
%      tune-short &\bf{45.87} & 49.84 & 50.36 & 48.96  \\
%      tune-mid   & 45.80 & \bf{50.22} & 50.70 & 49.25  \\
%      tune-long  & \bf {45.84} &\bf{ 50.24} &\bf{50.94} & \bf{49.42}  \\
      tune-short & 45.62     & 49.63     & 50.14     & 48.71  \\
      tune-mid   & 45.81 & \bf 50.20 & 50.71     & 49.27  \\
      tune-long  & \bf 45.84 & 50.17     & \bf 50.87 & \bf 49.35  \\

      \multicolumn{5}{l}{\bf PRO-fix}\\
%      tune-short & 45.86 & 50.01 & 50.51 & 49.14  \\
%      tune-mid & \bf{46.04*} & \bf{50.34*} & \bf{50.96*} & \bf{49.54*}  \\
%      tune-long & \it{44.02} & \it{48.07} & \it{48.71} & \it{47.54}  \\
       tune-short & 45.85     & 49.97     & 50.48     & 49.12 \\
       tune-mid   & \bf 46.06* & \bf 50.37* & \bf 50.98* & \bf 49.59* \\
       tune-long  & 45.68     & 50.04     & 50.61     & 49.20 \\
      \bottomrule

      \\\toprule
       \multicolumn{5}{l}{\bf  NIST Arabic-English (1-ref)}\\
       \multicolumn{5}{r}{\bf \it Average BLEU on unseen test sets}\\\cmidrule{2-5}

      & {\bf short} & {\bf mid} & {\bf long} & {\bf full} \\\midrule

      \multicolumn{5}{l}{\bf  MERT}\\
      tune-short & \bf 25.07 & 27.02     & 26.79     & 26.74  \\
      tune-mid   & 25.03     & 27.15     & 26.98     & 26.97  \\
      tune-long  & 25.04     & \bf 27.19 & \bf 27.15 & \bf 27.23  \\

      \multicolumn{5}{l}{\bf PRO-fix}\\
      tune-short & 25.04     & 26.98     & 26.75     & \bf 27.35*  \\
      tune-mid   & 25.09     & 27.19     & 27.09     & 27.23  \\
      tune-long  & \bf 25.10* & \bf 27.23* & \bf 27.16* & 27.28  \\
      \bottomrule

      \\\\\toprule
      \multicolumn{5}{l}{\bf WMT Spanish-English}\\
      \multicolumn{5}{r}{\bf \it Average BLEU on unseen test sets}\\\cmidrule{2-5}

      & {\bf short} & {\bf mid} & {\bf long} & {\bf full} \\\midrule
      \multicolumn{5}{l}{\bf  MERT}\\
%      tune-short & 24.50 & 25.59 & 27.46 & 26.70  \\
%      tune-mid & \bf{24.61*} & \bf{25.87*} & 27.78 & \bf{27.00}  \\
%      tune-long & 24.54 & \bf{25.87*} &\bf{27.90*} & \bf{27.05*}  \\
     tune-short & 24.53     & 25.65     & 27.53     & 26.79  \\
     tune-mid   & \bf 24.61* & 25.83 & 27.77     & 26.99  \\
     tune-long  & 24.52     & \bf 25.84* & \bf 27.88* & \bf 27.02  \\
     \multicolumn{5}{l}{\bf PRO-fix}\\

%     tune-short & \bf{24.54} & \bf{25.78} & \bf{27.83} & \bf{27.07*}  \\
%     tune-mid & 24.20 & 25.29 & 27.12 & 26.42  \\
%     tune-long & \it{22.82} & \it{23.96} & \it{25.74} & \it{25.08}  \\ \bottomrule
      tune-short & \bf 24.55 & \bf 25.78 & \bf 27.83 & \bf 27.07*  \\
      tune-mid   & 24.54 & 25.72 & 27.60 & 26.89  \\
      tune-long  & 24.52 & 25.66 & 27.59 & 26.84  \\
      \bottomrule
    \end{tabular}
    \caption{\label{tab:bleu}
%         A grid comparison of tuning and testing on all datasets.
         Average test BLEU scores when tuning on each \emph{short}/\emph{middle}/\emph{long} dataset,
         and testing on the remaining \emph{short}/\emph{middle}/\emph{long}/\emph{full} datasets.
%         Each cell represents the average over all relevant subsets (see example in the text).
%%         tuning on short/mddle/long subsets of the MT04/05/06/09,
%%         and testing on the same or different condition; similarly for the lower table, which uses Spanish-English.
%%         Translation results over different tuning/testing conditions.
%%         NIST v.13a BLEU score of tuning on a specific condition and testing on a different condition. Each cell of this table represents the average over all available datasets for tuning and their corresponding unseen counterparts for testing. For Arabic-English: NIST MT04, MT05, MT06, MT09. For Spanish-English: WMT newsiest 2008-2011.
%%         The best BLEU scores (at least 0.05 better) for each test condition are shown in \textbf{bold}.}
%         The best score for either MERT or PRO is bold;
%         the best overall score is marked with a $^*$.}
%%         scores that are considerably worse (-1.5 BLEU) than the best are in italic.}
%% On { \it italics} we present the subpar results, which are considerably worse (-1.5 BLEU) than the best.}
  \end{table}

There are several interesting observations that we can make about Table~\ref{tab:bleu}:

(1) Tuning on specific length condition does not necessarily yield the best results when testing on a similar condition.
This is surprising since it goes against the common wisdom that tuning datasets
should be as similar as possible to test-time input in terms of \emph{source side length}
or \emph{verbosity} (which are connected, as we saw in Section~\ref{sec:verb}).
This is especially true for PRO: for the same combination of language pair and number of references,
the best tuning dataset is the same regardless of whether testing on \emph{short}, \emph{middle} or \emph{long}.
For example, when testing on \emph{middle} sentences for Spanish-English, tuning on \emph{short} sentences
yields slightly better results compared to tuning on \emph{middle} sentences.
%MERT, on the other hand, tends to have better behavior in this respect, especially for Arabic-English:
%(i) with multiple references, tuning on \emph{middle}/\emph{long} is the best option when testing on \emph{middle}/\emph{long},
%and (ii) with a single reference, tuning on \emph{short}/\emph{long} is the best option when testing on \emph{short}/\emph{long}.

(2) MERT is consistently better when tuning on a \emph{long} dataset;
this is true across both language pairs and regardless of the number of references.

(3) PRO also has a general preference about what to tune on, but it depends on the \vb of the tuning set. I.e., PRO obtains the best parameters when tuning on the highest \vb sets.  This  depends on the combination of language pair and number of references (see Fig.\ref{fig:scatter}):
(i)~on Arabic-English with multiple references, it works best when tuning on \emph{middle},
(ii)~on Arabic-English with a single reference, it prefers tuning on \emph{long},
and
(iii)~on Spanish-English (single reference), it performs best when tuning on \emph{short}.

As we mentioned above, PRO tends to generate shorter translations \cite{nakov-guzman-vogel:2012:PAPERS},
and thus tuning on sentences with higher verbosity could compensate for this.
Figure~\ref{fig:scatter} shows that for the Arabic-English tuning dataset, longer sentences have higher verbosity.
Thus, better results should be expected when tuning on longer sentences,
especially in the case of a single reference, as (ii) indeed shows.
In the presence of multiple references,
the verbosity effect decreases to the extent that it becomes preferable to tune on middle sentences, as (i) shows.
In contrast, for Spanish-English, it is the shorter sentences that have higher verbosity,
and thus it is best to tune on short sentences, as (iii) indeed shows.

(4) PRO outperforms MERT on the Arabic-English dataset, regardless of the number of references, in all test sets. It also outperforms MERT in the full Spanish-English dataset, although not in specific conditions. The later effect can be attributed to the asymmetry in tuning conditions: The \emph{long} tuning set that MERT uses, has about four times more words than the \emph{short} set. Yet, PRO is able to obtain competitive results in such conditions. Thus, we conclude that it is possible to overcome the drawbacks of PRO, by choosing a higher verbosity dataset.

%\textbf{Do we want to discuss why (1)-(4) hold?}

%\textbf{Does tuning on some of the subsets improve over tuning on all?
%This is an important question! We might want to add results when tuning full to make this comparison.}


%(2) The general performance seems to be more specific to the choice of optimizer and the combination of language pair and number of references in the tuning/testing datasets. For instance, when testing on the full multi-reference Arabic-English set, tuning with MERT on long sentences (49.42 BLEU) and PRO on mid-length sentences (49.54 BLEU) yield the best results. However, PRO outperforms MERT in all testing conditions. For the single-reference Spanish-English datasets, MERT achieves the best results when tuning on longer sentences (except when testing on short). PRO achieves the best results when tuning on short sentences. MERT is better than PRO on specific length conditions, yet the performance of PRO is comparable to MERT's on the full-set condition (27.05 vs. 27.07).
%
%(3) Tuning on long sentences has a negative impact on PRO. This observation holds both on the full test sets of Arabic-English (loss of 1.6 BLEU) and Spanish-English (loss of 1.99 BLEU), as well as on the specific conditions. This suggests a potential problem with PRO's learning algorithm when faced with such types of input sentences.
%
%At this stage, it is difficult to assess whether the differences between the Arabic-English and the Spanish-English results stem from the nature of the language pair, or from the number of reference translations; we leave this question for future work.
%A different experimental procedure is required to distinguish such differences, which can be considered a future work.

%> fd<-full[full$set=="Ar-En"& full$tuner=="PRO",]



\subsection{Test vs. Tuning Verbosity and Source Length}

%Recently, there has been increased interest in the verbosity of MERT and PRO since it can affect automatic metrics such as BLEU \cite{nakov-guzman-vogel:2012:PAPERS}. Here, we explore how the observed verbosity in the test set varies depending on the characteristics of the tuning set.
% they behave with respect the input tuning sets.

In the previous subsection, we have seen that MERT and PRO
perform differently in terms of BLEU, depending on the characteristics of the tuning set.
Here, we study a different aspect: i.e. how they behave with respect to \emph{verbosity} and \emph{source side length}.

 \subsubsection{MERT -- Sensitive to Verbosity}

Figure~\ref{fig:tst_verb} shows a scatter plot of the tuning set \emph{verbosity} vs. the test \hvb when using MERT to tune under the different conditions,
and testing on each of the unseen full datasets.
Here, we chose to test only on full datasets only in order to avoid the \emph{verbosity} bias
that might occur for specific conditions (see Section~\ref{sec:verb}).

 \begin{figure*}[t!]
\centering
  \includegraphics[width=0.7\textwidth]{final.figure/tst_verb_ratio.pdf}

 \caption{\label{fig:tst_verb} Tuning set \emph{verbosity} vs. test \hvb when using MERT.
     Each point represents the result for an unseen test set, given a specific tuning condition.
%     On the left panel, we plot the results for the NIST Arabic-English datasets, and on the right panel, the results for the WMT Spanish-English datasets.
     The linear regressions shows the tendencies for each of the test-sets.
 }
 \end{figure*}

We can see in Figure~\ref{fig:tst_verb} strong positive correlation between the tuning set \emph{verbosity}
and the \hvb on the test datasets
The average correlation for the Arabic-English multi-reference is $r$=0.95, for the Arabic-English single-reference is $r$=0.98 and for the Spanish-English is $r$=0.97, which suggests that test \hvb of MERT is a function of the verbosity of the tuning set.
%We fit a linear regression model to each dataset and found significant correlation for the Arabic-English multi-reference
%and the Spanish-English datasets (with $p<0.00001$ for both).
In other words, MERT learns to generate a fixed proportion of words for each input source word.
%In this case, $0.65$  (90\% c.i. $[0.45,0.85]$) for Arabic-English and $0.66$ (90\% c.i. $[0.45,0.87]$) for Spanish-English.
This suggests that MERT tends to learn parameters that preserve the \emph{verbosity}:
lower \emph{verbosity} on the tuning set will yield test-time translations that are less verbose, and vice versa.

This can be explained by the fact that MERT optimizes corpus-level BLEU
and learns to output the ``right'' \emph{verbosity} on the tuning set.
%Yet, this makes it dependent on a parameter that we do not necessarily control or have access to beforehand:
%the length of the test references.

%While PRO is also sensitive to \emph{verbosity},
%this is minor compared to its sensitivity to the \emph{source-side sentence length}.
%it is positive for Arabic-English, but negative for Spanish-English.


\subsubsection{PRO -- Sensitive to Source Length}

In Figure \ref{fig:tst_len}, we plot the tuning set average \emph{source side length} vs. the testing hypothesis/reference \emph{length ratio} when using PRO to tune on \emph{short}, \emph{middle}, and \emph{long} and testing on each of the unseen full datasets, as in the previous subsection.


\begin{figure*}[t!]
 \centering
  \includegraphics[width=0.7\textwidth]{final.figure/tst_length_ratio.pdf}

 \caption{\label{fig:tst_len} Tuning set average \emph{source length} vs. test hypothesis/reference \emph{length ratio} for PRO.
     Each point represents the result for an unseen test set, given a specific tuning condition.
%     On the left panel, we plot the results for the NIST Arabic-English datasets, and on the right panel, the results for the WMT Spanish-English datasets.
     The linear regressions shows the tendencies across each of the test sets.
 }
 \end{figure*}

Figure \ref{fig:tst_len} shows that there is positive correlation between the tuning set average \emph{source side length} and the testing hypothesis/reference \emph{length ratio}.
For Spanish-English, this relationship is strong ($r$=0.64), and  for Arabic-English, this relationship is more clearly expressed with one reference ($r$=0.42),
than with multiple references, where the effect somewhat dampened ($r$=0.34).
%by the larger variance of the testing hypothesis/reference length ratios observed across the test sets.
The correlation is significant ($p<0.001$) when we take into account the contribution of the tuning dataset's \emph{verbosity} in the model.
This suggests that for PRO, both \emph{source length} and \vb influence the characteristics of the translations. I.e.
PRO learns the tuning dataset's \emph{verbosity}, much like MERT;
yet, the contribution of the length of the source sentences from the tuning dataset is not negligible.

For shorter tuning sentences, slightly shorter test translations are generated,
and longer tuning sentences yield longer test translations.

%For the single-reference Spanish-English datasets,
%the impact of the input sentence length is more pronounced ($p<0.0001$).
%We can see that tuning on shorter sentences yields translations that are slightly less verbose than the references.

%Tuning on longer sentences increases the \emph{verbosity} of the translations
%to the point that they become longer than the references.
%This might explain why tuning on shorter sentences is better for PRO with the Spanish-English datasets.

%MERT is also sensitive to \emph{source side length}, but the correlation is much lower;
%in fact, negative for both Arabic-English and Spanish-English.

Finally, note the ``stratification'' effect for the Arabic-English single-reference data.
We attribute this phenomenon to the differences across test datasets.

The same differences are attenuated for the Arabic-English multiple-reference datasets,
due to the \emph{effective reference length}.

%Also notice how tuning on longer sentences yields a ``shotgun'' type of unstable behavior.  The parameters obtained with these datasets are inconsistent, which leads to worse BLEU scores (both for Arabic-English and for Spanish-English). In the next section, we analyze this behavior in detail.

%Overall, for the multi-reference Arabic-English sets, PRO performs better than for Spanish-English. This might be due to the availability of multiple references or to the nature of the data itself; we leave this question for future work.
%To be able to solve this question effectively, we would have to tune on single-reference Arabic-English tuning sets and in multiple referenced Spanish-English datasets. Yet those experiments are outside the scope of this paper.

